Subfactors of index exactly 5

We give the classification of subfactor planar algebras at index exactly 5. All the examples arise as standard invariants of subgroup subfactors. Some of the requisite uniqueness results come from work of Izumi in preparation. The non-existence results build upon the classification of subfactor planar algebras with index less than 5, with some additional analysis of special cases.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> text/top_matter.tex <==
%!TEX root = ../exactly5.tex

\title{Subfactors of index exactly 5}

\author{Masaki Izumi}
%\address{
%}%
%\email{izumi@math.kyoto-u.ac.jp}

\author{Scott~Morrison}
%\address{
%}%
%\email{scott@tqft.net}

\author{David~Penneys}
%\address{
%}%
%\email{dpenneys@math.toronto.edu}

\author{Emily~Peters}
%\address{
%}%
%\email{epeters3@luc.edu}

\author{Noah~Snyder}
%\address{
%}%
%\email{nsnyder@gmail.com}

%\address{%
%\rm URLs: \tt \url{http://tqft.net/}\ \
%\url{http://math.toronto.edu/dpenneys}\\
%\  \tt \url{http://webpages.math.luc.edu/~epeters3/} \rm and \url{???}}


%\primaryclass{46L37} \secondaryclass{18D10} \keywords{
%  Planar Algebras, Subfactors
%}

